STANNIS: Low-Power Acceleration of Deep Neural Network Training Using Computational Storage

This paper proposes a framework for distributed, in-storage training of neural networks on clusters of computational storage devices. Such devices not only contain hardware accelerators but also eliminate data movement between the host and storage, resulting in both improved performance and power savings. More importantly, this in-storage processing style of training ensures that private data never leaves the storage while fully controlling the sharing of public data. Experimental results show up to 2.7x speedup and 69% reduction in energy consumption and no significant loss in accuracy.

==> reference.tex <==
@misc{  ref_int_domo, 
        title={Becoming A Data-Driven {CEO}}, 
        url={https://www.domo.com/solution/data-never-sleeps-6}, 
        journal={Domo}
    }
    
@misc{ref_int_AoI,
    title={Age of Information in Multiple Sensing},
    author={Alireza Javani and Marwen Zorgui and Zhiying Wang},
    year={2019},
    eprint={1902.01975},
    archivePrefix={arXiv},
    primaryClass={cs.IT}
}

@inproceedings{ref_int_cloud,
  title={Cloud hooks: Security and privacy issues in cloud computing},
  author={Jansen, Wayne A},
  booktitle={2011 44th Hawaii International Conference on System Sciences},
  pages={1--10},
  year={2011},
  organization={IEEE}
}


@article{ref_bck_allreduce,
  author  = {Alekh Agarwal and Oliveier Chapelle and Miroslav Dud\'{i}k and John Langford},
  title   = {A Reliable Effective Terascale Linear Learning System},
  journal = {Journal of Machine Learning Research},
  year    = {2014},
  volume  = {15},
  pages   = {1111-1133},
}



@misc{  ref_bck_ringallreduce, 
        title={Bringing {HPC} Techniques to Deep Learning}, 
        url={http://andrew.gibiansky.com/}, 
        
    }

@ARTICLE{ref_bck_benchmark,
       author = {{Wang}, Yu Emma and {Wei}, Gu-Yeon and {Brooks}, David},
        title = "{Benchmarking {TPU}, {GPU}, and {CPU} Platforms for Deep Learning}",
      journal = {arXiv e-prints},
     keywords = {Computer Science - Machine Learning, Computer Science - Performance, Statistics - Machine Learning},
         year = "2019",
        month = "Jul",
          eid = {arXiv:1907.10701},
        pages = {arXiv:1907.10701},
archivePrefix = {arXiv},
       eprint = {1907.10701},
 primaryClass = {cs.LG},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190710701W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@inproceedings{ref_bck_pytorch,
  title={Automatic Differentiation in {PyTorch}},
  author={Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and {DeVito}, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
  booktitle={NIPS Autodiff Workshop},
  year={2017}
}

@article{ref_bck_horovod,
  author    = {Alexander Sergeev and
               Mike {Del Balso}},
  title     = {Horovod: fast and easy distributed deep learning in {TensorFlow}},
  journal   = {CoRR},
  volume    = {abs/1802.05799},
  year      = {2018},
  archivePrefix = {arXiv},
  eprint    = {1802.05799},
  timestamp = {Mon, 13 Aug 2018 16:46:12 +0200}
  
  
}

@inproceedings{ref_bck_tensorflow,
  title={{Tensorflow}: A system for large-scale machine learning},
  author={Abadi  and others},
  booktitle={12th USENIX Symposium on Operating Systems Design and Implementation OSDI},
  pages={265--283},
  year={2016}
}



@article{ref_exp_facebook,
  author    = {Priya Goyal and
               Piotr Doll{\'{a}}r and
               Ross B. Girshick and
               Pieter Noordhuis and
               Lukasz Wesolowski and
               Aapo Kyrola and
               Andrew Tulloch and
               Yangqing Jia and
               Kaiming He},
  title     = {Accurate, Large Minibatch {SGD:} Training {ImageNet} in 1 Hour},
  journal   = {CoRR},
  volume    = {abs/1706.02677},
  year      = {2017},
  url       = {http://arxiv.org/abs/1706.02677},
  archivePrefix = {arXiv},
  eprint    = {1706.02677},
  timestamp = {Mon, 13 Aug 2018 16:49:10 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/GoyalDGNWKTJH17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{ref_exp_resnet,
  author    = {Kaiming He and
               Xiangyu Zhang and
               Shaoqing Ren and
               Jian Sun},
  title     = {Deep Residual Learning for Image Recognition},
  journal   = {CoRR},
  volume    = {abs/1512.03385},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.03385},
  archivePrefix = {arXiv},
  eprint    = {1512.03385},
  timestamp = {Wed, 17 Apr 2019 17:23:45 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/HeZRS15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{  ref_exp_tinyimgnt, 
        title={Tiny ImageNet Visual Recognition Challenge}, 
        url={https://tiny-imagenet.herokuapp.com/}, 
        
    }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%A Hitchhiker’s Guide On Distributed Training of Deep Neural Networks
@misc{chahal2018hitchhikers,
    title={A Hitchhiker's Guide On Distributed Training of Deep Neural Networks},
    author={Karanbir Chahal and Manraj Singh Grover and Kuntal Dey},
    year={2018},
    eprint={1810.11787},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}



%keras
@misc{chollet2015keras,
  title={Keras},
  author={Chollet, Fran\c{c}ois and others},
  year={2015},
  howpublished={\url{https://keras.io}},
}


@article{kim2016storage,
  title={In-storage processing of database scans and joins},
  author={Kim, Sungchan and Oh, Hyunok and Park, Chanik and Cho, Sangyeun and Lee, Sang-Won and Moon, Bongki},
  journal={Information Sciences},
  volume={327},
  pages={183--200},
  year={2016},
  publisher={Elsevier}
}

@article{park2016storage,
  title={In-storage computing for {Hadoop} {MapReduce} framework: Challenges and possibilities},
  author={Park, Dongchul and Wang, Jianguo and Kee, Yang-Suk},
  journal={IEEE Transactions on Computers},
  year={2016},
  publisher={IEEE}
}

@inproceedings{jun2015bluedbm,
  title={{Bluedbm}: An appliance for big data analytics},
  author={Jun, Sang-Woo and Liu, Ming and Lee, Sungjin and Hicks, Jamey and Ankcorn, John and King, Myron and Xu, Shuotao and others},
  booktitle={2015 ACM/IEEE 42nd Annual International Symposium on Computer Architecture (ISCA)},
  pages={1--13},
  year={2015},
  organization={IEEE}
}

@inproceedings{gu2016biscuit,
  title={{Biscuit}: A framework for near-data processing of big data workloads},
  author={Gu, Boncheol and et al.},
  booktitle={ACM SIGARCH Computer Architecture News},
  volume={44},
  number={3},
  pages={153--165},
  year={2016},
  organization={IEEE Press}
}

@inproceedings{ref_rltd_compstor,
    title={CompStor: An In-storage Computation Platform for Scalable Distributed Processing},
      author={Torabzadehkashi, Mahdi and Rezaei, Siavash and Alves, Vladimir and Bagherzadeh, Nader},
      booktitle={International Parallel and Distributed Processing Symposium Workshops (IPDPSW)},
      pages={1260--1267},
      year={2018},
      organization={IEEE}
}

@inproceedings{torabzadeh_HPCC,
  title={Accelerating HPC applications using computational storage devices},
  author={Torabzadehkashi, Mahdi and Heydarigorji, Ali and Rezaei, Siavash and Bobarshad, Hosein and Alves, Vladimir and Bagherzadeh, Nader},
  booktitle={21st International Conference on High Performance Computing and Communications},
  pages={1878--1885},
  year={2019},
  organization={IEEE}
}

@article{Torabzadeh_bigdata,
  title={Computational storage: an efficient and scalable platform for big data and HPC applications},
  author={Torabzadehkashi, Mahdi and Rezaei, Siavash and HeydariGorji, Ali and Bobarshad, Hosein and Alves, Vladimir and Bagherzadeh, Nader},
  journal={Journal of Big Data},
  volume={6},
  number={1},
  pages={100},
  year={2019},
  publisher={Springer}
}

@inproceedings{rezaei_ICCD,
  title={Scalable multi-queue data transfer scheme for FPGA-based multi-accelerators},
  author={Rezaei, Siavash and Kim, Kanghee and Bozorgzadeh, Eli},
  booktitle={36th International Conference on Computer Design (ICCD)},
  pages={374--380},
  year={2018},
  organization={IEEE}
}

@inproceedings{torabzadeh_PDP,
  title={Catalina: in-storage processing acceleration for scalable big data analytics},
  author={Torabzadehkashi, Mahdi and Rezaei, Siavash and Heydarigorji, Ali and Bobarshad, Hosein and Alves, Vladimir and Bagherzadeh, Nader},
  booktitle={27th Euromicro International Conference on Parallel, Distributed and Network-Based Processing (PDP)},
  pages={430--437},
  year={2019},
  organization={IEEE}
}
